Performance Improvement by Introducing Mobility in Wireless Communication Networks

Communication technology is a major contributor to our lifestyles. Improving the performance of communication system brings with various benefits to human beings. This report covers two typical such systems: wireless sensor networks and cellular networks. We study the influence of mobility in these networks. In wireless sensor networks, we consider the usage of mobile sinks to collect sensory data from static nodes. For the latter case, we design data collection protocols for a single mobile sink which aim at balancing the energy consumption among sensor nodes to improve the network lifetime. We also design an algorithm for multiple mobile sinks to collect urgent sensory information within the allowed latency. Regarding the mobility in cellular networks, we mean the service providers are mobile. Conventional approaches usually consider how to optimally deploy static base stations according to a certain metric, such as throughput. Base station densification is a solution, but it is not cost efficient. Introducing mobility is to let the base stations fly in the sky, resulting in less investment. We consider one of the key issues of using drones to serve cellular users: drone deployment. We have implemented all the proposed algorithms by either simulations or experiments, and the results have confirmed the effectiveness of these approaches.

==> chapter_agent.tex <==
\chapter{avoiding agent}
\minitoc
Safe mission planning in various threat environments is an important objective for military aircraft
such as strike aircraft, cruise missiles and Unmanned Aerial Vehicles (UAVs). Safe mission planning for such aircraft typically seeks to construct a route from origin to destination that minimizes the risk imposed by enemy threats. Typical examples include minimizing the risk of aircraft detection by radars or other ground sensors \cite{IMM04,ZAB1,BA1,BA2}, minimizing the risk of being destroyed by surface-to-air missiles \cite{KH03,MOR}, and minimizing exposure to radiation while passing through a contaminated area. 

This class of problems was studies in a number of  publications where two main approaches were proposed. The first approach is based on minimizing the cumulative threat exposure when flying through the threat environment \cite{KH03,ZAB2}. In the second approach, the objective is to minimize the probability of being detected \cite{BA1,BA2}. An alternative approach to safe military aircraft routing in threat environments is proposed in this paper. This approach is based on an optimization model where the objective is to  navigate an aircraft to its final destination while obtaining the shortest path that minimizes the threat level of the aircraft path. In some applications, this model is closer to reality. In particular, in Section \ref{S2} we consider the problem of minimizing worst case probability of being hit by one of several surface-to-air missiles which requires constructing an aircraft path minimizing the maximum threat level. In the proposed approach, regions with certain threat levels are treated as obstacles which the aircraft should avoid. Therefore, a part of the proposed solution is similar in spirit to the problem of safe robot navigation among obstacles; see e.g. \cite{lebeck13,agarwal16,solovey14, solovey15,MSHW15,MTS11,SH13,hoy2015algorithms} and references therein. The problem of finding the highly occluded paths on a terrain is considered in \cite{lebeck13}. Some models are similar to those used in this paper, such as the attenuated visibility map, which resembles our threat level function shown in Section \ref{S2}. The authors in \cite{agarwal16} consider the path planning problem amid obstacles for a point-wise robot, which aims at computing shortest path between two points while also maintaining a high clearance from the obstacles. The generated path is both the shortest and safe. They propose a polynomial-time approximation algorithm which guarantees the path length is at most $1+\varepsilon$ ($\varepsilon>0$) times of the optimal path. The problem of navigating a set of robots from start positions to goal positions in a planar environment cluttered with polygonal obstacles is studied in \cite{solovey14, solovey15} where the robots are modelled as unit-squares and unit-discs respectively. An algorithm is proposed in \cite{solovey15} which generates paths for the robots and the total length is at most $4n$ ($n$ is the number of robots) longer than that of the optimal paths. Similar to our work, the source and target should be sufficiently far from the threat agents.

The navigated aircraft considered in this paper is modelled as a Dubins car \cite{DUB57}, rather than a point robot \cite{agarwal16} or unit-square robots \cite{solovey14}. Such mathematical models are commonly applied to describe motion of ground robots as well as aerial or underwater vehicles moving in a horizontal plane \cite{MSHW15}. One advantage of the approach of this paper is in its computational simplicity. The proposed method results in construction of low-risk aircraft paths via a simple geometric procedure and does not require complex calculations. Unlike many existing publications on obstacle avoidance, the proposed method is based on rigorous mathematical analysis.

The remainder of the paper is organized as follows. Section \ref{S2} states the problem under consideration. Optimal aircraft paths that minimize the threat level  are described in Section \ref{S3}. Moreover, Section \ref{S3} contains the main theoretical result of the paper. Section \ref{Implementation} discusses the implementation of the proposed approach and provides the complexity analysis. Illustrative examples demonstrating the efficiency of the proposed method and comparisons with a fuzzy logic algorithm are presented in Section \ref{S4}. Finally, Section \ref{S5} presents a brief conclusion and suggestions for future research.

\section{Problem Statement}
\label{S2}
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
We consider an aircraft  or  a flying  robot moving in a plane and modelled as a Dubins car; see  \cite{DUB57}. It travels with a constant speed and is controlled by the angular velocity limited by a given constant. The model of the vehicle is as follows:

\begin{equation}
\label{1}
\begin{array}{l}
\dot{x}(t) = v \cos \alpha (t)
\\
\dot{y}(t) = v \sin \alpha (t)
\\
\dot{\alpha}(t) = u(t) \in [-u_M, u_M]
\end{array}, \qquad
\begin{array}{l}
x(0) = x_0
\\
y(0) = y_0
\\
\alpha(0) = \alpha_0.
\end{array} 
\end{equation}
Here $(x,y)$ is the vector of the Cartesian coordinates of the aircraft, the angle $\alpha$ describes its orientation, $v$ and $u$ are the speed and angular velocity, respectively. The maximal angular velocity $u_M$ is given. The aircraft satisfies the standard non-holonomic constraint 
\begin{equation}
\label{nonh}
|u(t)|\leq u_M
\end{equation} 
and the minimum turning radius of the aircraft is
\begin{equation}
\label{Rmin} R_{min}:= \frac{v}{u_M}.
\end{equation}
The non-holonomic model (\ref{1}) is widely used to describe planar motion of aircraft, UAVs, wheeled robots and missiles;
see e.g. \cite{MTS11,SH13,ST10,MS06,MSF08}. Any path $(x(t),y(t))$ of the aircraft (\ref{1}) is a planer curve 
satisfying the following constraint on its so-called average curvature (see \cite{DUB57}): let $Q(s)$ be this path parametrized by arc length, then
\begin{equation}
\label{ac}
\|Q'(s_1)-Q'(s_2)\|\leq \frac{1}{R_{min}}|s_1-s_2|.
\end{equation}
Here $\|\cdot\|$ denotes the standard Euclidean vector norm. Notice that we use the constraint (\ref{ac}) on average curvature because we cannot use the standard definition
of curvature from differential geometry (see e.g. \cite{POG}) since the curvature may not exist at some points of the  trajectory of the aircraft.

The initial position of the aircraft is in a known region ${\mathcal M}$. Also, there is a point-wise aircraft final destination ${\mathcal F}$ which also belongs to the region ${\mathcal M}$. There are $n$ steady point-wise  threat agents  in the plane with known coordinates $P_1=(x_1,y_1), P_2=(x_2,y_2),\ldots, P_n=(x_n,y_n)$. Each threat agent $i, 1\leq i\leq n$ has a known threat level continuous function $f_i(d)$ which describes the level of threat for a point at standard Euclidean distance $d\geq 0$ from  the threat agent $i$ located at $(x_i,y_i)$. In real life applications, threat agents can represent surface-to-air missiles or geophysical obstacles such as mountains or volcanoes from
which the aircraft needs to keep a safe distance.

We assume that the threat level functions $f_i(d)$ satisfy the following assumption.

\begin{Assumption}
\label{Ast} 
For any $i=1,2,\ldots,n$, there exists a constant $R_i>0$ such that $f_i(d)=0$ for all $d\geq R_i$,
 $f_i(d)>0$ for all $0\leq d< R_i$, and $f_i(d_1)>f_i(d_2)$ for all $0\leq d_1<d_2< R_i$.  Moreover, we assume that $R_i>R_{min}$ for all $i=1,2,\ldots,n$. A typical threat level function is shown in Fig. \ref{fig1}. Further, it is worth mentioning that this formulation is different from the conventional risk-theoretic function which monotonically increases with the distance.
\end{Assumption}

\begin{figure}[t]
\begin{center}
{\includegraphics[width=0.4\textwidth]{Fig/agent/fig1}}
\caption{A typical threat level function.}
\label{fig1}
\end{center}
\end{figure}

Moreover, we suppose that the region ${\mathcal M}$ satisfies the following assumption.

\begin{Assumption}
\label{As-1} The region ${\mathcal M}$ is a convex bounded closed set. The boundary $\partial D({\mathcal M})$ of the region ${\mathcal M}$ is a smooth curve with the curvature $k(p)$ at any point $p$ satisfying $k(p)\leq \frac{1}{R_{i}}$ for all $i=1,2,\ldots, n$.
\end{Assumption}

Assumption \ref{As-1} guarantees that the shape and the boundary of the region ${\mathcal M}$ are relatively simple.
This greatly reduces the complexity of the proposed navigation algorithm.

\begin{definition}\label{define_2_1}
A path $p(t)=(x(t),y(t))$ of the aircraft (\ref{1}) is said to be {\em reaching the final destination} if there exists a time $t_f>0$ such that $p(t_f) ={\mathcal F}$ and $p(t)$ belongs to the region ${\mathcal M}$ for all $i , t\in [0,t_f]$. Furthermore, $T[p(\cdot)]$ denotes the maximum threat level to which the aircraft was exposed on the path $p(\cdot)$:
\begin{equation}
\label{mtl}
T[p(\cdot)]:=\max_{i=1,2,\ldots,n,t\in [0,t_f]}f_i(d_i(t)) 
\end{equation}
where $d_i(t)$ is the distance between the aircraft and the threat agent $i$ at time $t$: 
\[
d_i(t):=\sqrt{(x(t)-x_i(t))^2+(y(t)-y_i(t))^2}.
\]
Moreover, $L[p(\cdot)]$ denotes the length of the path $p(\cdot)$.
\end{definition}


\begin{definition}
A reaching of the final destination path  $p_0(t)=(x_0(t),y_0(t))$ of the aircraft (\ref{1}) is said to be {\em optimal} if the following two conditions holds:
\begin{enumerate}
\item
For any other reaching of the final destination path $p(t)=(x(t),y(t))$, the inequality 
\begin{equation}
\label{E1}
T[p_0(\cdot)]\leq T[p(\cdot)]
\end{equation}
holds.
\item
If $T[p_0(\cdot)]= T[p_{*}(\cdot)]$ for some other reaching of the final destination path $p_{*}(t)=(x_{*}(t),y_{*}(t))$, then 
\begin{equation}
\label{E2}
L[p_0(\cdot)]\leq L[p_{*}(\cdot)].
\end{equation}
\end{enumerate}
If $p_0(t)$ is an optimal path, then  the number $T[p_0(\cdot)]$ is called the minimum achievable threat level.
\end{definition}

\begin{remark}
An optimal aircraft path guarantees the minimum possible
threat level. Moreover, among different paths with the same minimum threat level, the optimal path has a shortest length.
\end{remark} 

{\bf Problem statement:} Our problem is to design an optimal
aircraft path. In other words, the objective is to navigate the aircraft to the final destination ${\mathcal F}$ inside the region ${\mathcal M}$ while minimizing the maximum threat level and the length of the aircraft path.

{\bf Example: Minimizing worst case probability of being hit:} We introduce an example in which the optimal solution
requires minimizing the maximum threat level. Suppose that
the threat agents $P_1,P_2,\ldots,P_n$ are known ground locations from which surface-to-air missiles can be fired to hit the aircraft. Let $N$ be a total number of missiles. 
The probability of each missile to hit the aircraft depends on the distance $d$ between the aircraft and the agent from which the missile is fired and is described by a known function $f(d)$. The distribution of missiles between the threat agents $P_1,P_2,\ldots,P_n$  are not known to us. Our objective is to minimize the worst case (for all missiles distributions between the agents and all enemy firing strategies) probability that at least one of the $N$ missiles will hit the aircraft.

Let $[0,t_f]$ be the time interval during which the aircraft
moves from origin to destination, $d_i(t)$ be the distance
between the aircraft and the agent $i$ at time $t$. Furthermore, let
\[
d_{min}:=\min_{i=1,2,\ldots,n, ~~t\in [0,t_f]}d_i(t).
\]
It is obvious that for any aircraft path, the worst case scenario for us is when all $N$ missiles are fired from the closest agents at the moments when the aircraft is at the shortest distance $d_{min}$. In this case, the probability that the aircraft is hit by at least one missile is
\[
p_h=1-(1-f(d_{min}))^N=1-(1-\theta)^N
\]
where $\theta$ is the maximum threat level of the trajectory.
Therefore, the minimum possible value for the probability
$p_h$ is delivered by an aircraft path  with the minimum possible threat level $\theta$.


\section{Optimal Aircraft Path}
\label{S3}
In this section, we build optimal aircraft paths that minimize the threat level and the length.

\begin{notation}\label{notation_3_1}
In this paper, $d(w,h)$ denotes the standard Euclidean distance between the points $w$ and $h$. Moreover, 
$d(w,M)$ denotes the minimum  distance between the point $w$ and the closed set $M$.
\end{notation}

\begin{definition}\label{define_3_1}
Let $P_i$  be a threat agent such that the distance 
$d(P_i,\partial D({\mathcal M}))$ between $P_i$ and the boundary $\partial D({\mathcal M})$  of the region ${\mathcal M}$ satisfies $d(P_i,\partial D({\mathcal M}))<R_i$. Then it immediately follows from Assumption \ref{As-1}, that there exists a unique point $P_{*}$ at the  boundary of ${\mathcal M}$ such that  $d(P_i,\partial D({\mathcal M}))=d(P_i,P_{*})$. Then the point $P_{*}$ is called a critical point of type 1, and the number $\theta:=f_i(d(P_i,P_{*}))>0$ is called a critical threat level of type 1.
\end{definition}

\begin{definition}\label{define_3_2}
Let $P_i$ and $P_j$ be threat agents such that $d(P_i,P_j)<R_i+R_j$. Since the threat functions $f_i(\cdot), f_j(\cdot)$ are continuous and satisfy Assumption \ref{Ast}, there exists a unique point $P_{*}$ at the straight segment connecting $P_i$ and $P_j$ such that $f_i(d(P_i,P_{*}))=f_j(d(P_j,P_{*}))>0$. The point $P_{*}$ is called a critical point of type 2, and the number $\theta:=f_i(d(P_i,P_{*}))=f_j(d(P_j,P_{*}))>0$ is called a critical threat level of type 2.
\end{definition}

\begin{remark}\label{remark_3_1}
It is obvious that if $d(P_i,P_j)<R_i+R_j$ and the threat functions $f_i(\cdot)$ and $f_j(\cdot)$ are identical then the corresponding critical point $P_{*}$ is the middle of
the straight segment connecting $P_i$ and $P_j$.
\end{remark}

\begin{definition}
A number $\theta\geq 0$ is said to be a critical threat level
if one of the following conditions holds:
\begin{enumerate} 
\item 
$\theta =0$;
\item
$\theta$ is a critical threat level of type 1;
\item
$\theta$ is a critical threat level of type 2.
\end{enumerate}
Further, a point $P_{*}\in {\mathcal M}$ is said to be a critical point if it is either a critical point of type 1 or 
a critical point of type 2.
\end{definition}


Let $\theta\geq 0$ be a critical threat level. We now construct a non-convex closed set ${\mathcal M}(\theta)\subset {\mathcal M}$ as follows.
\begin{notation}
\label{note}
For any $i=1,2,\ldots,n$, introduce a radius $R_i(\theta)>0$ where $R_i(\theta):=R_i$ if $\theta =0$, and $R_i(\theta)$ satisfies $f_i(R_i(\theta))=\theta$ for $\theta>0$.
Notice that if $f_i(d)<\theta$ for all $d$, we do not introduce any $R_i(\theta)$. Now we construct the set ${\mathcal M}(\theta)$ by deleting from the region ${\mathcal M}$ all the open disks centred at the threat agents $P_i$ with the radius $R_i(\theta)$; see Fig. \ref{fig2}.
\end{notation}

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig2a}
        \caption{}
        \label{fig2a}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig2b}
        \caption{}
        \label{fig2b}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig2c}
        \caption{}
        \label{fig2c}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig2d}
        \caption{}
        \label{fig2d}
    \end{subfigure}
    \caption{Demonstration for constructing set ${\mathcal M}(\theta)$. (a) Initial figure with two agents locating at $P_1$ and $P_2$ with threat radius $R_1$ and $R_2$. (b) ${\mathcal M}(0)$. (c) ${\mathcal M}(\theta _1)$ by applying a critical point of type 2 and $\theta _1 =0.1$. (d) ${\mathcal M}(\theta _2)$ by applying a critical point of type 1 and $\theta _2 =0.3$.}\label{fig2}
\end{figure}  

It is clear that ${\mathcal M}(\theta)$ consists of all points ${\mathcal M}$ for which the threat level defined by
(\ref{mtl}) does not exceed $\theta$. It is also obvious that
${\mathcal M}(\theta_1)\subset {\mathcal M}(\theta_2)$ if 
$\theta_1\geq \theta_2$.

\begin{definition}
A critical threat level $\theta\geq 0$ is said to be 
a critical threat level with the connectivity requirement if
there exists a continuous curve belonging to ${\mathcal M}(\theta)$ and connecting the aircraft initial position $p(0)$ and the final destination ${\mathcal F}$. Moreover, a critical threat level $\theta$ with the connectivity requirement is called the minimum critical threat level with the connectivity requirement if the connectivity requirement does not hold for any critical threat level $\theta_{*}<\theta$.
\end{definition}

\begin{Assumption}
\label{Aso3-} 
Let $\theta$ be the minimum
critical threat level with the connectivity requirement.
We assume that $R_i(\theta)\geq R_{min}$ for all $i=1,2,\ldots,n$. 
\end{Assumption}

We also assume that the initial position $p(0)=(x(0),y(0))$ of the aircraft is far enough from the threat agents $P_1=(x_1,y_1), P_2=(x_2,y_2),\ldots, P_n=(x_n,y_n)$, the aircraft final destination ${\mathcal F}$ and the boundary of the region ${\mathcal M}$.
\begin{Assumption}
\label{Aso3} 
The following inequalities hold: $d({\mathcal F},p(0))> 8R_{min}$ and $d(P_i,p(0))> 8R_{min}+R_i$ for all $i=1,2,\ldots,n$. Finally, the distance between the aircraft initial position $p(0)$ and the boundary of the region ${\mathcal M}$ is greater than $8R_{min}$.
\end{Assumption}

Assumption \ref{Aso3} is a technical assumption that is necessary for the proof of our main theoretical result.

\begin{definition}
There are two circles with the radius $R_{min}$ that cross the initial aircraft position $p(0)$ and tangent to the aircraft initial heading $\alpha(0)$. We will call them the initial circles.
\end{definition}

\begin{definition}\label{define_3_6}
Let $\theta$ be the minimum critical threat level with the connectivity requirement. A straight line $S$ is said to be a tangent line if one of the following conditions holds:
\begin{enumerate}
\item
The line $S$ is simultaneously tangent to two circles centred
at $P_i$ and $P_j$ with radii $R_i(\theta)$ and $R_j(\theta)$, correspondingly, see Fig. \ref{fig3a} 
for an example.
\item
The line $S$ is simultaneously tangent to a circle centred
at $P_i$ with radius $R_i(\theta)$ and
an initial circle, see Fig. \ref{fig3b} 
for an example.
\item
The line $S$ is tangent to a  circle centred
at $P_i$ with radius $R_i(\theta)$ and crosses the final destination ${\mathcal F}$, see Fig. \ref{fig3c}
for an example.
\item
The line $S$ is tangent to an initial circle and crosses the final destination ${\mathcal F}$, see Fig. \ref{fig3d} 
for an example.
\end{enumerate}
\end{definition}

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.35\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig3a}
        \caption{}
        \label{fig3a}
    \end{subfigure}
    \begin{subfigure}{0.35\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig3b}
        \caption{}
        \label{fig3b}
    \end{subfigure}
    \begin{subfigure}{0.35\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig3c}
        \caption{}
        \label{fig3c}
    \end{subfigure}
    \begin{subfigure}{0.35\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig3d}
        \caption{}
        \label{fig3d}
    \end{subfigure}
    \caption{Demonstration for tangent lines. (a) Tangent lines between two circles centered at two agents. (b) Tangent lines between a circle centered at an agent and an initial circle. (c) Tangent lines between a circle centered at a agent and  ${\mathcal F}$. (d) Tangent lines between an initial circle and ${\mathcal F}$.}\label{fig3}
\end{figure}

\begin{definition}\label{define_3_7}
Points of circles centred at $P_i$ and initial circles belonging to tangent lines are called tangent points. 
\end{definition}

We consider only finite segments of tangent lines between tangent points such that their interiors do not cross
the interiors of the initial circles. Moreover, we consider
only finite segments of tangent lines between tangent points that belong to ${\mathcal M}(\theta)$.

\begin{definition}\label{define_3_8}
The vertices of the graph $\mathcal{G}(\theta)$ are the aircraft initial position $p(0)$, the final destination $\mathcal{F}$ and the tangent points. The edges of the graph $\mathcal{G}(\theta)$ are the tangent segments, arcs of the circles centred at $P_i$ with radii $R_i(\theta)$ and the initial circles that connect the vertices of the graph. The graph ${\mathcal G}(\theta)$ is called the extreme graph (see e.g. Fig. \ref{fig4a}).
\end{definition}

\begin{definition}\label{define_3_9}
A path connecting the aircraft initial position $p(0)$ and the final destination ${\mathcal F}$ on the extreme graph is said to be viable if the heading at the end of each edge of the path is equal to the heading at the beginning of the next edge of the path (see Fig. \ref{fig4b}).
\end{definition}

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig4a}
        \caption{}
        \label{fig4a}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig4b}
        \caption{}
        \label{fig4b}
    \end{subfigure}
    \caption{The extreme graph and the viable path. (a) An illustrative example of ${\mathcal G}(\theta)$ consisting of the vertices representing by the black solid points and the edges representing by the red solid lines and arcs. (b) $S_1$ is a viable path satisfying the heading constraint while $S_2$ and $S_3$ are not as they dissatisfy the heading constraint.}\label{fig4}
\end{figure} 

\begin{remark}
If a path connecting the aircraft initial position $p(0)$ and the final destination ${\mathcal F}$ on the extreme graph is viable it can be a path of the aircraft (since $R_{min}< R_i$ for all $i$, it follows from Assumptions \ref{Ast} and \ref{As-1} that any viable path on the extreme graph ${\mathcal G}(\theta)$ satisfies the curvature requirement (\ref{ac})). Also, it is obvious that if $\theta$ is the minimum critical threat level with the connectivity requirement then the corresponding critical point is a tangent point. The proposed procedure for constructing optimal paths reminds in spirit optimal path planning for ground vehicles in complex cluttered environments \cite{SH13}.
\end{remark}

Now we are in a position to present the main theoretical result of this paper.

\begin{Theorem}
\label{T1} Suppose that Assumptions~\ref{Ast}, \ref{As-1},
\ref{Aso3-} and \ref{Aso3} are satisfied. Then the following statements hold:
\begin{enumerate}
\item
The minimum achievable threat level $\theta$ is equal to the minimum critical threat level  with the connectivity requirement.
\item
If $\theta$ is the minimum critical threat level  with the connectivity requirement, then an optimal aircraft path is a shortest viable path on the extreme graph ${\mathcal G}(\theta)$.
\end{enumerate}
\end{Theorem}

{\bf The proof of Theorem \ref{T1}:} First, we prove that the minimum achievable threat level $\theta$ is equal to the minimum critical threat level  with the connectivity requirement. Indeed, as in \cite{DUB57}, it  follows from Ascoli's Theorem (see e.g. \cite{KF99}) that the minimum achievable threat level exists. Furthermore, it is obvious that  the minimum achievable threat level is a critical threat level. Furthermore, if some critical threat level $\theta_{*}$ does not satisfy  the connectivity requirement then it is obvious that there does not exist any path in ${\mathcal M}(\theta_{*})$ connecting the aircraft initial position $p(0)$ and the final destination ${\mathcal F}$. Therefore, the minimum achievable threat level $\theta$ cannot be less
than the minimum critical threat level with the connectivity requirement. On the other hand, we prove that if $\theta$ is  the minimum critical threat level, then the set ${\mathcal M}(\theta)$ contains  a shortest reaching the final destination path. Indeed, as in \cite{DUB57}, it follows from Ascoli's Theorem (see e.g. \cite{KF99}). Furthermore, we prove that this shortest reaching the final destination path is a shortest viable path on the extreme graph ${\mathcal G}(\theta)$. Indeed, let $S$ be a shortest (minimum length) reaching the final destination path. We now prove that the path $S$ does not go inside of any of two initial circles. Indeed, consider the circle $C$ of radius $6R_{min}$ centred at $p(0)$. Since $R_i(\theta) \leq R_i$ for all $i$, it follows from Assumption \ref{Aso3} that this circle is inside of the set ${\mathcal M}(\theta)$. Let $p_1$ be the point of the circle at which the path $S$ leaves this circle, and $\alpha_1$ be the trajectory heading at $p_1$. It means that $S$ consists of two segments $(p(0),p_1)$ and $(p_1,{\mathcal F})$ where $(p_1,{\mathcal F})$ is outside of the circle $C$. Now let $S_1$ be a path of minimum length connecting the points $p(0)$ and $p_1$ such that it has headings $\alpha(0)$ and $\alpha_1$ at these points, respectively, and the curvature requirement (\ref{ac}) is satisfied. It follows from the main result of \cite{DUB57} that such a path exists and $S_1$ belongs to the disk of radius $8R_{min}$ centred at $p(0)$. Therefore, Assumption \ref{Aso3} and the fact that $R_i(\theta) \leq R_i$ for all $i$ imply that $S_1$ is inside of the set ${\mathcal M}(\theta)$. Since, $S_1$ is a minimum length path, its length is less or equal to the length of $(p(0),p_1)$. On the other hand, the length of $(p(0),p_1)$ cannot be greater than the length of $S_1$ (if it is not true, then the path consisting of $S_1$ and $(p_1,{\mathcal F})$ would be a shorter   path reaching the final destination than $S$ which contradicts to our assumption that $S$ is a minimum length path. Hence, $(p(0),p_1)$ is a shortest path satisfying the curvature constraint (\ref{ac}). Therefore, it follows from the main result of \cite{DUB57} that $(p(0),p_1)$ consists of segments of two or less  minimum radius circles and a straight line segment and $(p(0),p_1)$ does not cross the interiors of the both  initial circles. Hence, we have proved that that the path $S$ does not go inside of any of two initial circles.

\begin{figure}[t]
\begin{center}
{\includegraphics[width=0.45\textwidth]{Fig/agent/fig5}}
\caption{If a segment of a path is not a straight line segment, lies outside of the initial circles and does not cross the boundary of $\mathcal M(\theta)$, then there exists a shorter path.
}
\label{fig5}
\end{center}
\end{figure}

Now let $S_2$ be a minimum length path inside of the set ${\mathcal M}(\theta)$ connecting the points $p(0)$ and ${\mathcal F}$ which is not crossing two initial circles. Now we do not assume that $S_2$ satisfies condition (\ref{ac}). Since we have proved that the path $S$ does not go inside of any of two initial circles, the length of $S_2$ is less or equal to the length of $S$. Now we prove that $S_2$ consists of segments of the boundaries of the set ${\mathcal M}(\theta)$ and two initial circles, and straight line segments connecting two different points on these boundaries. Indeed, we prove it by contradiction. If this statement does not hold, then there exists a point $p_2\in S_2$ which is outside of  two initial circles and the boundary of the set ${\mathcal M}(\theta)$, and $p_2$ is not an interior point of a straight line segment of $S_2$. In this case, in some small neighbourhood of $p_2$ we can replace the segment of path $S_2$ containing $p_2$ by a straight line segment which does not intersect two initial circles and the boundary of the set ${\mathcal M}(\theta)$; see Fig. \ref{fig5}. Therefore, we can construct a path with shorter length than $S_2$ satisfying all the requirements. Furthermore, it follows from Theorem 5 of \cite{LA92} that any straight line segment of $S_2$ connects either two tangent points or a tangent point and the final destination point. Hence, the path $S_2$ may consist of segments of two initial circles, segments of the boundary of the set ${\mathcal M}(\theta)$ and segments of straight lines connecting tangent points or a tangent point and the target. Therefore, the path $S_2$ is a viable path on the extreme graph ${\mathcal G}(\theta)$. Finally, since $R_i(\theta) \leq R_i$ for all $i$, it follows from Assumptions \ref{Ast} and \ref{As-1} that any viable path on the extreme graph ${\mathcal G}(\theta)$ satisfies the curvature requirement (\ref{ac}). This completes the proof of Theorem \ref{T1}.

\section{Implementation and Complexity Analysis}\label{Implementation}

In this section, we describe the implementation of the proposed navigation and present the complexity analysis.

\subsection{Implementation}\label{imp}
The input of our algorithm includes $p(0)$, $\mathcal{F}$, $P_i$, $R_i$, $f_i$ and $\partial D(\mathcal{M})$. Note $i=1,...,n$. The output is the minimum threat level and the shortest path. The overall procedure is outlined below:
\begin{enumerate}
\item Compute all the critical points and the corresponding threat levels; the sets of them are represented by $CP$ and $\Theta$ respectively;
\item Sort the critical points according to the ascending of threat level (without introducing more notations, $CP$ and $\Theta$ denote the sorted sets henceforce); let $k=1$;
\item Using $CP(k)$ to construct the corresponding non-convex set $\mathcal{M}(\Theta(k))$ and then the extreme graph $\mathcal{G}(\Theta(k))$;
\item Check whether $\mathcal{G}(\Theta(k))$ satisfies the connectivity requirement; if yes, output $\Theta(k)$ and the shortest path, and exit; otherwise, $k=k+1$ and repeat Step 3).
\end{enumerate}

According to Definition \ref{define_3_1} and \ref{define_3_2}, Step 1) requires the following information as input: $P_i$, $f_i$, $R_i$ and $\partial D(\mathcal{M})$. To calculate the critical points of type 1, we need to check whether an agent's threat range crosses the region boundary according to Notation \ref{notation_3_1}. Following Definition \ref{define_3_1}, the critical points of type 1 are the points on the region boundary which are the closest points to the related agents, see e.g. Fig. \ref{fig2}. To calculate the critical points of type 2, we need to check whether two agents' threat range overlap. 

We specify the threat level function $f_i(d)$ and threat radius $R_i(\theta)$ for all $i=1,...,n$ as follows:
\begin{equation}\label{eq3}
f_i(d)=
\begin{cases}
1-\frac{d}{R_i},\ \ 0\leq d < R_i \\
0,\ \ \ \ \ \ \ \ \ d \geq R_i \\
\end{cases}
\end{equation}
\begin{equation}\label{eq4}
R_i(\theta)=R_i\cdot(1-\theta)
\end{equation}
It is obvious the proposed piecewise linear threat level functions satisfy all the requirements of  Assumption \ref{Ast}. 

Considering Remark \ref{remark_3_1}, i.e., the threat functions are identical, the critical points of type 2 are the middle points of the connection of the related two agents, see e.g. Fig. \ref{fig2}. In the situation of non-identical threat functions, the critical point of type 2 is not the middle point. Details of computing such critical point are presented in Appendix \ref{AppendixB}. The algorithm to compute critical points and threat levels is given in Algorithm \ref{cp}. Here we assume $n>1$. If $n=1$, the critical points of type 2 do not exist. In this case, there are at most two critical points of type 1. Then, Line 3 of Algorithm \ref{cp} should be slightly modified by finding two $P_*$ on different sides, see e.g., Fig. \ref{fig9a}.

\begin{algorithm}[t]
\caption{Compute critical points and threat levels}\label{cp}
\begin{algorithmic}[1]
\Require $P_i$, $R_i$, $\partial D(\mathcal{M})$, $f_i$ 
\Ensure $CP$, $\Theta$
\State $CP\leftarrow \emptyset$, $\Theta \leftarrow \emptyset$
\For{$i=1:n$}
\State Find $P_*$ on $\partial D(\mathcal{M})$ such that $d(P_i,P_*)$ is minimized 
\If {$d(P_i,P_*)<R_i$}
\State Add $P_*$ to $CP$; add $f_i(d(P_i,P_*))$ to $\Theta$
\EndIf
\For{$j=i+1:n$}
\If {$d(P_i,P_j)<R_i+R_j$}
\State Compute $P_*$ by either $\frac{P_i+P_j}{2}$ or Eq. (\ref{cp_coordinates})
\State Add $P_*$ to $CP$ and the corresponding threat level to $\Theta$
\EndIf
\EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

Step 2) sorts the critical points according to the threat levels. The idea behind is that if a smaller threat level leads to an extreme graph satisfying the connectivity requirement, there is no need to check the larger levels.

In Step 3), we build up the non-convex set $\mathcal{M}(\Theta(k))$ and then construct the extreme graph $\mathcal{G}(\Theta(k))$ based on the selected critical point $CP(k)$. To construct $\mathcal{G}(\Theta(k))$, we need to construct all the tangent lines according to Definition \ref{define_3_6}. There are two types of tangent lines between: 1) a circle and a point outside; and 2) two circles, both of which can be precisely computed. The formulations of common tangent lines for these two cases are given in Appendix \ref{AppendixC}. 

In Step 4), we need to verify whether $\mathcal{G}(\Theta(k))$ meets the requirement of connectivity by Breadth First Search (BFS) \cite{BFS}. If connected, the algorithm BFS can also figure out the shortest path from $p(0)$ to $\mathcal{F}$. We finally check whether the heading requirement is satisfied by all two successful edges. If we can obtain a viable path under the current threat level, then it is the minimum threat level and the path is the optimal one; otherwise, we need to test the next critical point which leads to a larger threat level, i.e., repeat Step 3).

\subsection{Complexity analysis}\label{complexity_analysis}
Now we analyse the complexity of the proposed algorithm.

Shown as Algorithm \ref{cp}, the time complexity of Step 1) is $O(n^2)$. For the sorting procedure, many algorithms can be finished with time complexity lower than $O(n^2)$, e.g., Heapsort, which is in $O(n\log(n))$. Both of Step 1) and 2) will be executed by only once.

We point out that our minimum threat level and the shortest path will be found within a finite number of rounds. This number equals to the size of $CP$. We first consider an extreme case to estimate the upper bound of $|CP|$ and then analysis the complexity of applying BFS in Step 4). 

Since any pair of agents have at most one critical point of type 2, the maximum number of critical points of type 2 is $\frac{n(n-1)}{2}$. Since any agent has at most one critical point of type 1 with the boundary, the maximum number of critical points of type 1 is $n$. So $|CP|$ is upper bounded by $\frac{n(n+1)}{2}$. 

As discussed in Section \ref{imp}, the tangent lines can be calculated analytically (the time complexity is $O(1)$). Any pair of circles can have up to four tangent lines, and there are at most two tangent lines between $\mathcal{F}$ and a circle. There are $n+2$ circles in the graph. In the extreme case, i.e., any agent circle has four common tangent lines with all the other circles, the number of tangent lines is $4C_{n+2}^2-4$. Note the tangent lines between two initial circles should be taken out. Between the $n$ threat circles and $\mathcal{F}$, there are $2n$ tangent lines. Thus, the total number of tangent lines is $2n^2+6n+2n$. The total number of tangent points in the graph is $2(2n^2+6n)+2n$. Note, the 2 here corresponds to the fact that there are two tangent points for the tangent line between the circles; while for the tangent line between the threat circles and $\mathcal{F}$, only the tangent points on the circles should be considered. Besides, using BFS to check the connectivity of $\mathcal{G}(\Theta(k))$ results in the time complexity of $O(n^2)$. 

Overall, in the extreme case, the time complexity of our algorithm is $O(n^2+nlog(n)+\frac{n(n+1)}{2}\times n^2)=O(n^4)$. 

However, we also point that the extreme case does not exist in real applications. In our considered scenario, the agents should be well placed. In other words, not any two agents can have common tangent lines. Besides, not all agents' threat areas overlap with the region boundary. Thus, the upper bound of $|CP|$ will be decreased significantly. Here, we consider at most $K$ (a constant) threat circles overlap with each other simultaneously. In this case, number of critical points of type 2 is at most $Kn/2$ and that of critical points of type 1 is no larger than $n$. Thus, the upper bound of $|CP|$ is reduced from $O(n^2)$ to $O(n)$. Further, the numbers of vertices and edges in $\mathcal{G}(\Theta(k))$ is decreased accordingly, both from $O(n^2)$ to $O(n)$.

Therefore, in general, the complexity of our algorithm is $O(n^2)$ instead of $O(n^4)$. In the next section, we will use some simulation to demonstrate the complexity difference between the extreme and general cases.

\section{Simulation Results}
\label{S4}

This section presents examples to demonstrate the efficiency of the proposed method. We first set up the simulation environment. Then, we present the simulations for identical threat radius and non-identical threat radii. Finally, we compare the proposed approach with a fuzzy logic algorithm.

We consider several scenarios and build optimal paths of the aircraft. The aircraft initial heading to the X-axis is $\alpha(0)=\pi$. The speed of the aircraft is set as $v=1.5m/s$ and its maximum angular velocity is $u_M=0.5rad/s$. $R_i$ is taken as $12m$ for Simulation 1, 2, 3 and 4, and $30m$ for Simulation 5. There is only one agent in Simulation 1 and 2, i.e., $n=1$, while $n=2,\ 6,\ 10$ for Simulation 3, 4 and 5 respectively. 
\subsection{Identical threat radius}
Fig. \ref{fig8} demonstrates a scenario where $\mathcal{M}$ is wide enough and the aircraft is able to reach the final destination with $0$ threat level. However in Fig. \ref{fig9}, the aircraft cannot arrive at the final destination with 0 threat level. In this case, the optimal path crosses a critical point of type 1. Another simulation where the optimal path crosses a critical point of type 2 is shown in Fig. \ref{fig10}.  A complex simulation is displayed in Fig. \ref{fig11}. 
 Six agents block the region and the aircraft arrives at its final destination with 0.08 threat level. A more challenging simulation is shown in Fig. \ref{fig12} where the maximum threat level is 0.10. In these cases, the optimal paths contain critical points of type 2.

\begin{figure}[t]
\begin{center}
{\includegraphics[width=0.45\textwidth]{Fig/agent/fig8}}
\caption{Simulation 1. $\theta=0.00$.}
\label{fig8}
\end{center}
\end{figure}

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig9a}
        \caption{}
        \label{fig9a}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig9b}
        \caption{}
        \label{fig9b}
    \end{subfigure}
    \caption{Simulation 2 for crossing the critical point of type 1. (a) $\theta=0.00$. (b) $\theta=0.06$.}\label{fig9}
\end{figure}  

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig10a}
        \caption{}
        \label{fig10a}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig10b}
        \caption{}
        \label{fig10b}
    \end{subfigure}
    \caption{Simulation 3 for crossing the critical point of type 2. (a) $\theta=0.00$. (b) $\theta=0.07$.}\label{fig10}
\end{figure}  

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig11a}
        \caption{}
        \label{fig11a}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig11b}
        \caption{}
        \label{fig11b}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig11c}
        \caption{}
        \label{fig11c}
    \end{subfigure}
    \caption{Simulation 4 with 6 agents. (a) $\theta=0.00$. (b) $\theta=0.02$. (c) $\theta=0.08$.}\label{fig11}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig12a}
        \caption{}
        \label{fig12a}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig12b}
        \caption{}
        \label{fig12b}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig12c}
        \caption{}
        \label{fig12c}
    \end{subfigure}
    \caption{Simulation 5 with 10 agents. (a) $\theta=0.00$. (b) $\theta=0.09$. (c) $\theta=0.10$.}\label{fig12}
\end{figure}

Now we test the complexity analysis in Section \ref{complexity_analysis} on Simulation 3, 4 and 5, where $n$ = 2, 6 and 10. We summarize the actual numbers of critical points, vertices and edges in the extreme graph in Table \ref{table:number}. Furthermore, we provide the estimated numbers of critical points, vertices and edges for both the general case and the extreme case. For the general case, considering the actual environment, $K$ takes 2, 2 and 3 respectively for Simulation 3, 4 and 5. As seen in Table \ref{table:number}, the estimations in the general case is more closer to reality than the extreme case.

\begin{table}[t]
\begin{center}
\caption{The number of critical points, vertices and edges}\label{table:number} 
  \begin{tabular}{| c | c | c | c | c|}
    \hline
    \multicolumn{2}{|c|}{} & $CP$ & Vertex & Edge\\ \hline
    \multirow{4}{*}{$n=2$} & Round 1& \multirow{2}{*}{3}& 10& 9\\
    \cline{4-5} 
    & Round 2& & 13&17\\ 
    \cline{2-5}
    & General & 3& 38&55\\
    \cline{2-5}
    & Extreme&3& 54&78\\ \hline
    \multirow{5}{*}{$n=6$} & Round 1& \multirow{3}{*}{9}& 24&26 \\ 
    \cline{4-5} 
    & Round 2& & 26&30\\ 
    \cline{4-5} 
    & Round 3& & 29&37\\
    \cline{2-5}
    & General& 12& 78& 115\\
    \cline{2-5}
    &Extreme& 21& 246&366\\ \hline
    \multirow{5}{*}{$n=10$} & Round 1& \multirow{3}{*}{12}& 96& 121\\ 
    \cline{4-5} 
    & Round 2& & 118&154\\ 
    \cline{4-5} 
    & Round 3& & 125&171\\
    \cline{2-5}
    & General& 25&166&247\\
    \cline{2-5}
    & Extreme& 55&566&846\\ \hline
    \end{tabular}
\end{center}
\end{table}

\subsection{Non-identical threat radii}\label{S52}
We further execute simulations for the case of non-identical threat radii. In Simulation 4, the threat radii of the six agents are 12, 13, 12, 12, 11 and 10 meters respectively. In Simulation 5, the threat radii are 30, 28, 26, 30, 32, 31, 29, 27, 30 and 28 meters respectively. The results are demonstrated in Fig. \ref{fig13} and \ref{fig14}. 
Since the threat radii have been changed, correspondingly the achieved threat levels of passing the region are also different: 0.03 in Simulation 4 and 0.05 in Simulation 5. 

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig13a}
        \caption{}
        \label{fig13a}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig13b}
        \caption{}
        \label{fig13b}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig13c}
        \caption{}
        \label{fig13c}
    \end{subfigure}
    \caption{Simulation 4 with 6 agents and non-identical threat radii. (a) $\theta=0.00$. (b) $\theta=0.02$. (c) $\theta=0.03$.}\label{fig13}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig14a}
        \caption{}
        \label{fig14a}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig14b}
        \caption{}
        \label{fig14b}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig14c}
        \caption{}
        \label{fig14c}
    \end{subfigure}
    \caption{Simulation 5 with 10 agents and non-identical threat radii. (a) $\theta=0.00$. (b) $\theta=0.03$. (c) $\theta=0.05$.}\label{fig14}
\end{figure}

\subsection{Comparison with existing work}
\begin{figure}[h]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig15a}
        \caption{$R(\theta)=9.2$m.}
        \label{fig15a}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig15b}
        \caption{$R(\theta)=8$m; threat level: 0.145; path length: 118.3m.}
        \label{fig15b}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig15c}
        \caption{$R(\theta)=7$m; threat level: 0.086; path length: 117.2m.}
        \label{fig15c}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig15d}
        \caption{$R(\theta)=6$m; threat level: 0.290; path length: 108.0m.}
        \label{fig15d}
    \end{subfigure}
    \caption{Comparison between our approach and the fuzzy logic algorithm on Simulation 4.}\label{fig15}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig16a}
        \caption{$R(\theta)=27$m.}
        \label{fig16a}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig16b}
        \caption{$R(\theta)=20$m; threat level: 0.261; path length: 407.3m.}
        \label{fig16b}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig16c}
        \caption{$R(\theta)=15$m; threat level: 0.325; path length: 373.6m.}
        \label{fig16c}
    \end{subfigure}
    \begin{subfigure}{0.45\textwidth}
        \includegraphics[width=\textwidth]{Fig/agent/fig16d}
        \caption{$R(\theta)=10$m; threat level: 0.191; path length: 389.3m.}
        \label{fig16d}
    \end{subfigure}
    \caption{Comparison between our approach and the fuzzy logic algorithm on Simulation 5.}\label{fig16}
\end{figure}

This subsection presents the comparison with a fuzzy logic approach. Fuzzy logic has been used in autonomous vehicle navigation to avoid collisions with obstacles, see e.g., \cite{llorca2011fuzzy, al2014fuzzy}. Since we use the Dubins car model to describe the motion of the aircraft, we have only one output of fuzzy logic system, i.e., angular velocity. We take front distance, left-front distance, right-front distance, distance to destination, and angle difference between the aircraft's current heading and the destination angle as inputs. Such system requires the aircraft to measure distances and know its current location.

Before applying the fuzzy logic algorithm to our problem, it is worth mentioning that such fuzzy logic algorithm requires at least one valid path from origin position to destination in the region. If we regard the threat regions with radii $R_i$ as obstacles, the field is blocked. Since the fuzzy logic system is unable to find the best threat level, we simply start from the radius corresponding to the minimum threat level found by our proposed approach, and then test some smaller radii.

We apply the fuzzy logic algorithm to Simulation 4 and 5, and the generated paths are displayed in Fig. \ref{fig15} and \ref{fig16} respectively. For the sake of comparison, the paths by our approach are also displayed. In Fig. \ref{fig15a}, the threat radius is 9.2m, which is consistent with the obtained 0.08 threat level. The fuzzy logic system fails to find a path leading the aircraft from initial position to destination. Further, we test the radii of 8, 7, and 6m, and the generated paths are demonstrated in Fig. \ref{fig15b}, \ref{fig15c} and \ref{fig15d}. We observe from these simulations that the best path generated by the fuzzy logic system is in Fig. \ref{fig15c}, whose threat level is 0.086 and path length is 117.2m. But this is still worse than our path, whose threat level and path length are respectively 0.080 and 112.1m. We execute the same procedure for Simulation 5. The best path generated by the fuzzy logic system is in Fig. \ref{fig16}, whose threat level is 0.191 and path length is 389.3m. Again the path produced by our proposed approach outperforms in threat level (0.100) and path length (365.6m).

Through these simulations we find that the threat level of a path generated by fuzzy logic system is uncontrollable. In contrast, our approach is based on a rigorous mathematical analysis and is guaranteed to find the optimal threat level from a finite set of candidates. Further, the length of the paths produced by our approach is proved to be the shortest under the threat level. The presented simulation results show  that our approach achieves better performance than the fuzzy logic algorithm  in terms of both threat level and path length.

\section{Conclusion and Future Research}
\label{S5}
In this paper, we proposed an optimization model where the objective is to navigate an aircraft or a flying robot to its final destination while minimizing the maximum threat level and the length of the aircraft path. The construction of optimal paths involves a simple geometric procedure and is very computationally efficient. The effectiveness of the proposed method has been demonstrated by illustrative examples and  comparisons with existing work. It should be pointed out that this paper considers a 2D or planar navigation problem. An important direction of future research will be an extension of the presented planar algorithm to practically important cases of 3D threat environments.
